SelectFormer: Private and Practical Data Selection for Transformers

Critical to a free data market is $\textit{private data selection}$, i.e. the model owner selects and then appraises training data from the data owner before both parties commit to a transaction. To keep the data and model private, this process shall evaluate the target model to be trained over Multi-Party Computation (MPC). While prior work suggests that evaluating Transformer-based models over MPC is prohibitively expensive, this paper makes it practical for the purpose of data selection. Our contributions are three: (1) a new pipeline for private data selection over MPC; (2) emulating high-dimensional nonlinear operators with low-dimension MLPs, which are trained on a small sample of the data of interest; (3) scheduling MPC in a parallel, multiphase fashion. We evaluate our method on diverse Transformer models and NLP/CV benchmarks. Compared to directly evaluating the target model over MPC, our method reduces the delay from thousands of hours to tens of hours, while only seeing around 0.20% accuracy degradation from training with the selected data.

==> design.tex <==
% !TeX root = main.tex
%\section{\sys{} Overview}
\section{Method}
\label{sec:design}

\subsection{High-level workflow}

\xzlNote{need a workflow figure}

The model owner has to specify a selection number. The data owner has to preprocess \xzlNote{meaning what} the data. Both parties then set up the secure computation framework, and the secrete share, which reveals no information about the real data, for both the data points as well as the model are shared across the parties. 

\xzlNote{missing details}
\begin{itemize}
\item the target model? the proxy model? how are they initialized
\item before selection, purchase 5\%, why? for what purpose...
\item rank based on entropy... 
\item (what info is leaked) intentional
\end{itemize}

Selection often takes several phases to facilitate the whole process. More lightweight proxy models will be used first to filter out irrelevant data, while more accurate, heavyweight proxy models used in later phases to pinpoint high-value data. 


For example, if the model owner wants to select the top 15\% instance. The whole selection can be divided into three phases. The first phase ranks the top 50\% using a model with only 2 heads and hidden size 2. The Second phase ranks the top 30\% using a model with 6 heads and hidden size 8. In the final phase, the parties rank the top 15\% using the vanilla proxy model.

\xzlNote{use proxy model to query...}

The data is being processed in a batched fashion. 
\xzlNote{how do batches work in this picture}
The scheduler, given the scenario and operator costs, regroups the instance and distributes them to a specific task.

\xzlNote{through this process, what info is leaked, what is not}

%$ ------------------ might be useful to a system paper ----------------
\begin{comment} 
\subsection{System Architecture}

There are three main components in the system. One is the proxy model $M_p$ which, has a smaller architecture than the target model $M_t$. Next is the secure computation framework which provides these secure machine-learning computations. Lastly is our scheduler. Given the cost of the operations, the bandwidth, and memory usage, the scheduler will regroup the instances and assign them to the tasks to maximize the throughput.

\input{fig-approxarch}


\subsection{Deployment}

Our system can be deployed in all sorts of server-edge communications. We offer the possibility to exploit the vast amount of data stored in edge devices, which a great amount has no labels and contain private information.

Another application is direct to medical records. A large number of medical records are being kept private and oftentimes, the data is imbalanced and not labeled. Our system can help the medical model owner to secretly select the most valuable data points for training. 

\subsection{Applicability}

Although our system has a wide range of applications, we want to stress several things we observed.

(1) Our system deals with the threat model the same as the secure framework being used. Common framework work in semi-honest setting which assumes all the players will follow the protocols and will not deviate from the playbook.

(2) We assume the dataset is unlabeled, which is common in real-world scenarios. With labeled datasets, there are other selection techniques can be applied, e.g., influence function, which is more costly. 

(3) Our method is not only applied to transformers but also to other neural network architectures like CNN and RNN. (some ablation study / related work can be used here?)

\paragraph{Application}

\paragraph{System environment}

\paragraph{Scenarios}

\end{comment} 

==> fig-approxarch.tex <==
% !TeX root = main.tex

\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/placeholder-ApproxProxyArch.pdf}
	%	\vspace{-2em}
	\caption{The system architecture of \sys{}. Our core parts are colored as navy. The rest of modules is already in the existing self-driving. XXX FL: need to show layernorm XXX}
	\label{fig:design:overview}
	
	%	\vspace{-5mm}
\end{figure}

==> fig-crypten-nn-dag.tex <==
% !TeX root = main.tex

\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/fig_MM_DAG.png}
        %	\vspace{-2em}
        \includegraphics[width=0.48\textwidth]{figs/fig-analysis-Comm.png}
        \includegraphics[width=0.48\textwidth]{figs/fig-analysis-compu.png}
	%	\vspace{-2em}
	\caption{Matrix Multiplication DAG}
	\label{fig:design:crypten-analysis}
	%	\vspace{-5mm}
\end{figure}

==> fig-decomposition.tex <==
\begin{figure}[ht]
	\centering
	\includegraphics[width=1\textwidth]{figs/Decomposition.jpg}
	%	\vspace{-2em}
	\caption{Beavor triple decomposition}
	\label{fig:design:decomposition}
	%	\vspace{-5mm}
\end{figure}

==> fig-dynamic-batching.tex <==
\begin{figure}[ht]
	\centering
	\includegraphics[width=1\textwidth]{figs/fig-dynamic-batching.png}
	%	\vspace{-2em}
	\caption{stacking cheap blocks to reduce the communication latency. Here \sys{} identify the ReLU and the following linear layers to be latency-bound. After the first linear layers, \sys{} set synchronization barriers. After all batches go through the first linear operation, \sys{} regroup all data and send them to the next opeation.}
	\label{fig:design:dynamic batching}
	%	\vspace{-5mm}
\end{figure}

==> fig-module-analysis.tex <==
\begin{figure}[t]
	\centering
        \begin{minipage}[t]{0.48\linewidth}
            \centering
          \includegraphics[width=\linewidth, height=3cm]{figs/fig-module-analysis-cropped.pdf}
        \end{minipage}\hfill
        \centering
        \begin{minipage}[t]{0.48\linewidth}
            \centering
          \includegraphics[width=\linewidth]{figs/fig-batch-co-execution-cropped.pdf}
        \end{minipage}\hfill

 
	%	\vspace{-2em}
	\caption{Commmunication bound modules v.s Latency bound modules. The Layernorm activation, the following linear projection, and the entropy modules are latency-bound. This is because they have relatively small input shape}
	\label{fig:design:module analysis}
	%	\vspace{-5mm}
\end{figure}

==> fig-mpccost.tex <==
% !TeX root = main.tex

\begin{figure}[ht]
	% \centering
	% \includegraphics[width=1\textwidth]{figs/fig-techniques-runtime-cropped.pdf}
	% %	\vspace{-2em}
	% \caption{Runtime of applying different techniques (in hours). For BERT and DistilBERT, we use ImbSST2, which has 41743 data points. For ViT and ViT-small, we use ImbCifar10, which has 9995 data points.}
	% \label{fig:design:multi}
	% %	\vspace{-5mm}

\begin{figure*}[ht]
	
  \centering
  \begin{minipage}[t]{0.25\linewidth}
    \includegraphics[width=\linewidth]{figs/fig-e2e-BERT.pdf}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.25\linewidth}
  	\includegraphics[width=\linewidth]{figs/fig-e2e-DistilBERT.pdf}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.25\linewidth}
  	\includegraphics[width=\linewidth]{figs/fig-e2e-ViT.pdf}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.25\linewidth}
  	\includegraphics[width=\linewidth]{figs/fig-e2e-ViT-small.pdf}
  \end{minipage}\hfill
   \begin{minipage}[t]{1\linewidth}
   	  \centering
  	\includegraphics[width=0.3\linewidth]{figs/fig-e2e-legend-cropped.pdf}
  \end{minipage}
  \caption{
  Run time for models to select on different datasets. % as shown by driving scores.
\sys{} achieves around two-order of magnitude of speedup.
}
  \label{fig:eval:e2e}
\end{figure*}
 
\end{figure}

==> fig-multiphase-acc.tex <==
% !TeX root = main.tex
\begin{table}[t]
	\centering
	\includegraphics[width=\textwidth]{figs/multiphase-acc.pdf}
%	\vspace{-2em}
	\caption{Multi-phase selection is able to significantly reduce runtime and maintain comparable performance. On QQP, three-phase selection achieves 9.5\% higher accuracy than using one phase.
	main results: 16, (2,16), (2,8,16)}
	\label{tab:gridsearch}
%	\vspace{-2em}
\end{table}

==> fig-overview.tex <==
% !TeX root = main.tex

%%%% Figure 
\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{figs/placeholder-overview.pdf}
	%	\vspace{-2em}
	\caption{An overview of our design (XXX liked this model XXX need to improve incrementally)}
	\label{fig:intro:overview}
	%	\vspace{-5mm}
\end{figure}
%%%%%

==> impl.tex <==
% !TeX root = main.tex

\section{Implementation}
\subsection{Attention Mask Value}
On NLP tasks, maximum length padding and truncation are necessary because of varying sentence lengths. It is ideal for these paddings to be negative infinity but attention layers often use a large negative number in the attention mask to mask them out. However, very large negative numbers will cause the data underflow problem on Crypten and dominate the attention input results in approximation MLPs degradation. \cite{chen-etal-2022-x} recommends the optimal range of attention mask is between -2 and -5, hence we set the mask value to -3.




==> motiv_copy.tex <==
\section{Background}
\label{sec:motiv}
% \input{fig-overview}

%\subsection{System model}
\subsection{Assumptions on systems}

\paragraph{Two parties}
The model owner possesses a pretrained Transformer model \target{} and wants to finetune it. 
The data owner owns the dataset $D$ for selection. 
The model owner is interested in buying $b$ datapoints ($b<|D|$) from dataset $D$ which will be used to finetune the model $M_t$. 
The model owner has a private, small validation set, on which she wants to maximize the test accuracy. 
The two parties agree on $b$ and that they will use MPC for selection. 

% We consider the following setting. One data owner who owns the dataset $D$ for selection. One model owner who owns the target model $M_t$. The data owner has $n$ datapoints. The owner of model is interested in buying $m$ datapoints ($m<n$) which will be used to train the model $M_t$. Intuitively, the model owner is interested in the $m$ datapoints, which would yield the highest accuracy gain after training model $M_t$ on all of them. 


% We assume both parties know some metadata before the selection. (e.g. number of data points, model architecture,  preprocessing pipelines, etc.)

% (Optionally, the model owner wants to estimate the accuracy gain before making the purchase decision).  -- maybe don't include this part

\paragraph{Datapoints}
We follow a common premise in prior work on data selection: \cite{coleman2019selection}, \cite{Mullapudi2021LearningRareCategory}, \cite{Mahmood2022OptimizingDataCollection}, 
the dataset $S$ is unlabeled and might have an imbalanced class distribution, which warrants careful selection before training. 
This premise is motivated by real-world situations where data labels are scarce
and data owners often lack the motivation, expertise, and authority to label their data \cite{Hoi2006MedicalImage}, \cite{Smith2018LessIsMore}. 

\paragraph{Threat model}
Without alternation, we follow a semi-honest model widely used in prior security research (\cite{knott2021crypten}, \cite{dong2023puma}, \cite{mohassel2017secureml}): 
both parties faithfully follow the MPC 
protocol but nevertheless attempt to learn each other's private information (model weights and datapoints $S$) through their interactions. 
Notably, we do not deviate from protocols implemented by well-known frameworks such as Crypten. 
As such, our privacy guarantee is as strong as the underlying framework. 

\subsection{Algorithm framework}

\paragraph{Foundations}
Our selection is based on prediction entropy and proxy models. 
(1) Maximum entropy selection roots in Active Learning (AL) \cite{pengzhen2020activelearningsurvey} \cite{Settles2012Activelearning} \cite{David1994TrainingTextClassifiers}: 
selecting from unlabeled data to maximize training performance. 
To appraise an example $x$ for training model $M$, 
AL runs a forward pass of $M$ over $x$ (or query $x$ with $M$) and computes the prediction entropy: 
higher entropy implies lower model confidence, hence higher learning value of $x$. 
(2) Proxy models reduce selection overhead. 
Querying all examples in $D$ with $M_t$ can be slow. 
To this end, prior work uses a lightweight model $M_p$ called ``proxy'' for selection before  training $M_t$ with the selected data~\cite{coleman2019selection}. 
To select valuable data, $M_p$'s prediction should resemble that of $M_t$; 
hence $M_p$ is often created as a miniature version of $M_t$: 
examples include ResNet-18 as proxy for ResNet-50 \cite{coleman2019selection}. 
We follow the ideas to use as proxy models Transformers with fewer layers and attention heads. 

\paragraph{Our algorithm} 
Given a target model $M_t$ ($n$ layers with $m$ heads), dataset $D$, and budget $b$. We first randomly purchase 5\% data from the data owner as a sample and call it bootstrap data $s$. It's important for the model owners to have a certain level of understanding of the data candidates before committing to a deal.
Then we prepare proxy models run on MPC. We take the bottom layers (closest to input) from $M_t$ to get $M_p$: $M_p = M_t'$. Then we train $M_p$ on $s$. Its input distributions of nonlinear modules will be used to train approximation MLPs. We augment training data by generating the same distribution data.
Multi-phase selection requires a different proxy model in each phase. To get the proxy model $M{p1}$ in phase 1, we prune $M_p$ to just one layer and one most important head out of $n$ layers and $m$ heads. Then we replace non-linear modules with our MLPs. It is the same for other proxy models, without pruning. Each $M_{pi}$ now has different pairs of approximation MLPs, having larger hidden dimensions in the later phase.
Next, we will query each proxy model and go through each phase by the order over MPC. The selection sets to identify $b$ examples with the highest prediction entropy: $E(x) = -\sum^n_{i=1} p(x_i) \log p(x_i)$ across all the data class $i$. The earlier phase will browse more data and retain a smaller portion of candidates for the latter phase. The last phase will retain $b-s$ data. Together with bootstrap data $b$, we have fulfilled our budget $b$. 
% The (optional) appraisal is done by computing the average prediction entropy of the selected examples: \xzlNote{add formula:}
% \xzlNote{add formula:}
\textcolor{blue}{Issue: how do we get labels for the bootstrap??? maybe saying we are using AL setting since they also require a small portion of labels}

% The selection sets to identify $b$ examples with highest prediction entropy: \xzlNote{add formula:}





\begin{comment}
Data selection is a major part of Active Learning(AL). AL aims to select the most valuable data from unlabeled data that maximizes the model performance. It assumes that most data points are unlabeled 
(except for a small fraction of labeled data for bootstrapping training). 

\paragraph{Data Selection Metric -- Entropy}
Entropy is often used in depicting the state of disorder, but it can also be used to measure how confident the model is about the data sample. Intuitively, if the model is confident with which class the input sample should belong to, we should expect that the sum of all classes' entropy will be very small and they are not very important to the model. Therefore, filtering these data would not have a big difference in the final model performance.

Forward pass loss is also a very common and useful signal for evaluating how confident the model is about the input data. However, we choose entropy maximum selection because we are targeting imbalanced and unlabeled clients' data. Hence entropy is a natural decision as losses cannot be computed. 
Maximum entropy data selection has been widely used by prior Active Learning(AL) works. But model training and data selection are intertwined together and need to browse all the input data with the large target model, which makes this paradigm impractical under MPC settings.
More importantly, calculating entropy requires no data labels. While other works like using an influence function need labels to get losses.
\end{comment}




\begin{comment}
To reduce the selection cost, prior works proposed to use of a lightweight model as the "proxy model" to do the data selection and train the target model with the selected data eventually. 
% Even using proxy models, data selection over MPC is prohibitively expensive. 
% A top reason is that nonlinear arithmetic, which incurs high cost when performing over MPC, is pervasive in building blocks of modern DNNs. 
% Take attention mechanisms, the key building block of BERT and ChatGPT, as an example: each column is an attention matrix is computed via softmax, 
% which comprises max, exponential, and reciprocal. 
A common practice of selecting data both economically and accurately is filtering by a small proxy model which has the same architecture as the target model but fewer layers\cite{coleman2019selection}. Similarly, we use a small transformer model as the proxy to do the selection for a large target transformer model. Different models can all be used as our target model, but transformer models are the cutting-edge and mainstream models in both NLP and CV research nowadays. Hence we do experiments on 4 kinds of transformer variants.
There are even cheaper machine learning models that can be used as proxies. But we want to take advantage of powerful attention mechanisms to maintain good selection performance. Besides, the same architecture proxy models would have similar selection preferences as their large target model. 
\end{comment}




\subsection{An overhead analysis: transformer over MPC}
\xzlNote{owned by Changhong}

% \input{fig-crypten-analysis}

% \input{fig-crypten-nn-dag}

\paragraph{Transofmers}
We focus on transformer \cite{Ashish2017transformer} encoder-based models, which consist of multiple encoder layers stacked together. Each encoder layer comprises a Multihead attention module and a Feed Forward Network module. Both modules are followed by a layer norm and residual connection. The Multihead attention module consists of a QKV linear operation, the attention operation, and an attention-out operation. The attention operation has a softmax function which requires lots of computational power. The Feed Forward Network module includes a linear operation, an activation operation followed by a linear operation. 

% For $l$-th layer input $H^i \in \mathbf{R} ^ {s \times h}$, where $s$ is the sequence length, $h$ is the hidden state size. $H^i$ will first go through the multi-head attention module, where the inputs of query, key, and value are $H^i$ itself. In the multi-head attention, there are $N_h$ attention heads. For each head, query, key, and value are linearly projected into different sub-spaces. The projected query and key are multiplied and normalized to compute the score. If there is padding, the mask function will apply to the score matrix. The score matrix is then applied to the softmax function and multiplied with the projected value to calculate the attention. Afterward, the attention of all heads is concatenated and projected back to the hidden state size $h$. Finally, the output will add the value input and is applied with layer norm. This ends the multi-head attention module. The encoder architecture only has one multi-head attention module while the encoder architecture has two multi-head attention modules back to back. The attention module is followed by the feed-forward network module, where the input is linearly projected into a bigger space, activated, and linearly projected into the original space. This ends the $l$-th layer. 

\paragraph{2PC} \ 
% In the MPC system, the model owner will input the model and the data owner will input the dataset. In the MPC system, all the numbers will be split into multiple shares and distributed across all parties.

We assume secret sharing under the 2PC setting \cite{Qiang20192PC}. Under 2PC, suppose the model owner inputs $x$, and the data owner inputs $y$. The model owner will randomly split $x$ into two shares $x_1$ and $x_2$ ($x_1 + x_2  = x$). The model owner will hold $x_1$ and send the data owner $x_2$. Similarly, the data owner will split $y$ into $y_1$ and $y_2$ and send $y_2$ to the model owner ($y_1 + y_2  = y$). If two parties want to recover a number, they can send their share to each other and add them up. The shares don't reveal any information about the numbers as they are randomly generated.

In order to compute $z = x + y$. Both parties add their respective shares of $x$ and $y$. The new shares become $z_1 = x_1 + y_1$ and $z_2 = x_2 + y_2$. The two parties can recover $z = z_1 + z_2$. For multiplication, parties need to generate random triple $a$, $b$, and $c$ ($ab = c$) called Beavor triple. Like $x$ and $y$, $a$, $b$, and $c$ are split and distributed across parties. The model owner will compute $\epsilon_1 = x_1 - a_1 $, $\delta_1 = y_1 - b_1$ while the data owner will compute $\epsilon_2 = x_2 - a_2 $, $\delta_2 = y_2 - b_2$. Then the two parties have to perform a communication to recover $\epsilon$ and $\delta$. Model owner then compute $z_1 = c_1 + \epsilon y_1 + \delta x_1 + \epsilon \delta$. The data owner computes $z_2 = c_2 + \epsilon y_2 + \delta x_2$. This way $z = x * y = z_1 + z_2$. During the whole process, all these intermediate results including $\epsilon_1$, $\epsilon_2$, $\delta_1$ and $\delta_2$ does not reveal any information about $x$, $y$ and $z$.



\paragraph{Major Overheads} \xzlNote{add figures}

Similar to the popular framework Crypten \cite{knott2021crypten}, we assume the MPC system uses two secret sharing schemes: arithmetic and binary \cite{Goldreich1987secretshare} \cite{Damgard2011secretshare}. The major limitation comes from the incompatibility with the non-linear functions. For example, it's extremely expensive or impossible to perform functions such as softmax, logarithmic, and exponential. To resolve this, MPC systems have to design approximation functions that are still expensive to use. In Figure XXX, we examine the cost of the operations for a transformer block on Crypten. We measure the cost per instance.

We have the following observations.

(1) The cost of nonlinear arithmetic dominates, coupled with the large hidden size. Out of all the modules, nonlinear arithmetic contributes 161 (93.6\%) communication rounds and 2.64GB (84.6\%). 
As mentioned above, this is because MPC needs to approximate nonlinear arithmetic with linear operations. 
The approximation is typically iterative (e.g. Newton Ralpson... Tylor series expansions) which requires a large number of rounds.
Hence, nonlinear arithmetic should receive high attention in optimization. 

(2) Bandwidth bound vs. latency bound. 
Some modules require lots of data exchange in a small number of communication rounds. 
This is because they have high internal parallelism. 
Examples include matrix multiplication of Q and K. 
By contrast, some modules perform many communication rounds, each exchanging low data. 
This is particularly pronounced after logits are calculated and the number of model activations greatly shrinks. 
Examples include XXX which uses iterative guess to approximate nonlinear operations.
The observation leaves an opportunity for executing the two types of modules -- for different datapoints -- in parallel and hide the communication latency. 

% Assuming the MPC framework uses two secret sharing schemes: arithmetic and binary. The major overheads come from two functions: multiplication and comparison. Multiplication in MPC often employs Beavor Triples, which is a pair of randomly generated numbers. Parties need to send intermediate results to others to complete the operation. Similarly, the comparison operations require transforming the arithmetic secrets into binary secrets, which need multiple rounds of communications. 

% Furthermore, since directly computing functions like exponential and logarithms are extremely expensive or not even possible, many frameworks have to use approximations such as limit approximation, Newton-Raphson iteration, and Yao’s Garbled Circuits. As shown in the Figure, as non-linear functions commonly resides in the transformer architecture, they introduces tremendous overheads. 

% First, multiplication in MPC adds communication. Unlike addition, multiplications in MPC often lead to multiple rounds of communication. Meanwhile, matrix multiplications are all over the machine learning models. To this end, systems have to employ Beavor Triples, which is a pair of randomly generated numbers, to improve communication efficiency.

% %  Limitation 2 on top of limitation 1, shorter discussion on 1

% Second, The non-linear functions often introduce tremendous overhead. MPC doesn't support non-linear functions such as exponential, division, and square root which are commonly existed in machine learning modules. Current systems try to approximate these functions using limit approximation, Newton-Raphson iteration, and Yao’s Garbled Circuits. But previous results have shown that all these approximations add an enormous amount of commutation as well as computation. 

% We choose Crypten \xzlNote{cite}, a popular framework for MPC. 


% Figure \ref{fig:design:crypten-analysis} shows the cost breakdown by modules in a transformer. 

% computation analysis on softmax & layernorm


% (1) Some operations require more communication while others require more bandwidth. Take computing the key, value, and query as an example. It requires 34MB and 5.8 GFLOPs. Meanwhile, computing the Attention requires 12.5MB \xzlNote{only 12MB?} and 14GFLOPs. Both operations take a single round.
% (maybe fuse with 3)
% \xzlNote{the point is quite off. need to compare computation vs. communication. }

% is the major bottleneck. 
% All modules require computation of XXX-XXXX GFLOPs; 
% which, even on mobile/embedded computers can be finished in XXX seconds (numbers estimated from XXX). 
% By contrast, the required communication is high, 
% XXX-XXX rounds and XXX--XXX giga bytes. 
% The required delays will range from XXX -- XXX seconds on typical wired and wireless Internet conditions. 
% The communication delays are XXX orders of magnitude higher than the computation delays. 
% In our subsequent analysis and design, we focus on communication overhead. 


% \xzlNote{may be go to sec2?? merge}
% Matrix multiplication of $[A]$ and $[B]$ comprises a sequence of operations:
% exchange of $[A - X]$ and $[Y - B]$ (where $[X]$ and $[Y]$ are randomly generated)
% (network bandwidth bound), computing of $[X][Y]$ (compute bound), 
% and getting the decrypted result $\epsilon$ and $\delta$, and calculate $[A][B] = [X][Y] + \epsilon[Y] + \delta[X] + \epsilon\delta$ (compute bound); 
% ReLU is bound to network latency (one real-valued input requires 9 communication rounds and only 464 bytes); 
% comparison is bound to network latency (a comparison of two real values requires 8 rounds and an exchange of only 864 bytes). 



%(4) The memory consumption is higher than normal model execution. Dealing with secret share instead of normal data takes more operations. Especially when arthritic share converts to binary shares. The Carryout adder circuit often takes a huge amount of memory. If memory is insufficient, crypten compromise with another circuit which take more communication data and communication rounds.
%\xzlNote{how much higher? need some numbers}



==> scripts/Makefile <==
# batch convert all .pptx files in a directory to .pdf  
# files and crop them. 
# 
# to be used in conjunction with ppt.vbs, which converts
# a .pptx file into a pdf. 
#
# usage: copy this file and ppt.vbs to figs/ and run make
# there
#
# environment: win 10 cmd
#

docobjects := $(patsubst %.docx,%.pdf,$(wildcard *.docx)) $(patsubst %.dox,%.pdf,$(wildcard *.dox))
pptobjects := $(patsubst %.pptx,%.pdf,$(wildcard *.pptx))

current_dir  := $(shell cd)

all : check_overlap $(docobjects) $(pptobjects) 

	
docx : $(docobjects)

pptx : $(pptobjects)

clean :
	del /Q $(docobjects) $(pptobjects)

check_overlap :
	@echo "$(current_dir)"
		
		
%.pdf.uncrop : %.docx
	"c:\Windows\SysWOW64\cscript.exe" "$(scriptDir)\docx.vbs" "$(current_dir)\$^" "$(current_dir)\$@"

%.pdf.uncrop : %.dox
	"c:\Windows\SysWOW64\cscript.exe" "$(scriptDir)\docx.vbs" "$(current_dir)\$^" "$(current_dir)\$@"

%.pdf.uncrop : %.pptx
	"c:\Windows\SysWOW64\cscript.exe" "$(scriptDir)\ppt.vbs" "$(current_dir)\$^" "$(current_dir)\$@"

%.pdf: %.pdf.uncrop
	"$(scriptDir)\bin\pdfcrop.exe" $^ $@
	
	
.PHONY: check_overlap all docx pptx

==> scripts/bin/pdfcrop <==
#!/usr/bin/env perl
use strict;
$^W=1; # turn warning on
#
# pdfcrop.pl
#
# Copyright (C) 2002, 2004, 2005, 2008-2012 Heiko Oberdiek.
#
# This program may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.2
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.2 or later is part of all distributions of LaTeX
# version 1999/12/01 or later.
#
# See file "README" for a list of files that belong to this project.
#
# This file "pdfcrop.pl" may be renamed to "pdfcrop"
# for installation purposes.
#
my $prj         = 'pdfcrop';
my $file        = "$prj.pl";
my $program     = uc($&) if $file =~ /^\w+/;
my $version     = "1.38";
my $date        = "2012/11/02";
my $author      = "Heiko Oberdiek";
my $copyright   = "Copyright (c) 2002-2012 by $author.";
#
# Reqirements: Perl5, Ghostscript
# History:
#   2002/10/30 v1.0:  First release.
#   2002/10/30 v1.1:  Option --hires added.
#   2002/11/04 v1.2:  "nul" instead of "/dev/null" for windows.
#   2002/11/23 v1.3:  Use of File::Spec module's "devnull" call.
#   2002/11/29 v1.4:  Option --papersize added.
#   2004/06/24 v1.5:  Clear map file entries so that pdfTeX
#                     does not touch the fonts.
#   2004/06/26 v1.6:  Use mgs.exe instead of gswin32c.exe for MIKTEX.
#   2005/03/11 v1.7:  Support of spaces in file names
#                     (open("-|") is used for ghostscript call).
#   2008/01/09 v1.8:  Fix for moving the temporary file to the output
#                     file across file system boundaries.
#   2008/04/05 v1.9:  Options --resolution and --bbox added.
#   2008/07/16 v1.10: Support for XeTeX added with new options
#                     --pdftex, --xetex, and --xetexcmd.
#   2008/07/22 v1.11: Workaround for open("-|").
#   2008/07/23 v1.12: Workarounds for the workaround (error detection, ...).
#   2008/07/24 v1.13: open("-|")/workaround removed.
#                     Input files with unsafe file names are linked/copied
#                     to temporary file with safe file name.
#   2008/09/12 v1.14: Error detection for invalid Bounding Boxes.
#   2009/07/14 v1.15: Fix for negative coordinates in Bounding Boxes
#                     (David Menestrina).
#   2009/07/16 v1.16: Security fixes:
#                     * -dSAFER added for Ghostscript,
#                     * -no-shell-escape added for pdfTeX/XeTeX.
#   2009/07/17 v1.17: Security fixes:
#                     * Backticks and whitespace are forbidden
#                       for options --(gs|pdftex|xetex)cmd.
#                     * Validation of options --papersize and --resolution.
#   2009/07/18 v1.18: * Restricted mode added.
#                     * Option --version added.
#   2009/09/24 v1.19: * Ghostscript detection rewritten.
#                     * Cygwin: `gs' is preferred to `gswin32c'.
#   2009/10/06 v1.20: * File name sanitizing in .tex file.
#   2009/12/21 v1.21: * Option --ini added for IniTeX mode.
#                     * Option --luatex and --luatexcmd added for LuaTeX.
#   2009/12/29 v1.22: * Syntax description for option --bbox fixed
#                       (Lukas Prochazka).
#   2010/01/09 v1.23: * Options --bbox-odd and -bbox-even added.
#   2010/08/16 v1.24: * Workaround added for buggy ghostscript ports
#                       that print the BoundingBox data twice.
#   2010/08/26 v1.25: * Fix for the case that the PDF file contains
#                       an entry /CropBox different to /MediaBox.
#                     * \pageinclude implemented for XeTeX.
#                     * XeTeX: --clip does not die, but this option
#                       is ignored, because XeTeX always clip.
# 2010/08/26 v1.26: * XeTeX's \XeTeXpdffile expects keyword
#                     `media', not `mediabox'.
#                   * New option --pdfversion.
#                     Default is `auto' that means the PDF version
#                     is inherited from the input file. Before
#                     pdfcrop has used the TeX engine's default.
#                   * Option --luatex fixed (extra empty page at end).
# 2010/09/03 v1.27: * Workaround of v1.24 fixed.
# 2010/09/06 v1.28: * The Windows registry is searched if Ghostscript
#                     is not found via PATH.
#                   * Windows only: support of spaces in command
#                     names in unrestricted mode.
# 2010/09/06 v1.29: * Find the latest Ghostscript version in registry.
# 2010/09/15 v1.30: * Warning of pdfTeX because of \pdfobjcompresslevel
#                     avoided when reducing \pdfminorversion.
#                   * Fix for TeX syntax characters in input file names.
# 2010/09/17 v1.31: * Passing the input file name via hex string to TeX.
#                   * Again input file names restricted for Ghostscript
#                     command line, switch then to symbol link/copy
#                     method.
# 2011/08/10 v1.32: * Detection for gswin64c.exe added.
# 2012/02/01 v1.33: * Input file can be `-' (standard input).
# 2012/04/18 v1.34: * Format of --version changed
#                     from naked version number to a line with
#                     program name, date and version.
# 2012/10/15 v1.35: * Additional debug infos added for Perl version.
# 2012/10/16 v1.36: * More error codes added.
# 2012/10/16 v1.37: * Extended error messages if available.
#                   * Fix for broken v1.36.
# 2012/11/02 v1.38: * Fix for unsufficient cleanup, if function `cleanup' is
#                     prematurely called in `eval' for `symlink' checking.

### program identification
my $title = "$program $version, $date - $copyright\n";

### error strings
my $Error = "!!! Error:"; # error prefix

### make ENV safer
delete @ENV{qw(IFS CDPATH ENV BASH_ENV)};

# Windows detection (no SIGHUP)
my $Win = 0;
$Win = 1 if $^O =~ /mswin32/i;
$Win = 1 if $^O =~ /cygwin/i;
use Config;
my $archname = $Config{'archname'};
$archname = 'unknown' unless defined $Config{'archname'};

### extended error messages
sub exterr () {
    chomp(my $msg_errno = $!);
    chomp(my $msg_extended_os_error = $^E);
    if ($msg_errno eq $msg_extended_os_error) {
        $msg_errno;
    }
    else {
        "$msg_errno/$msg_extended_os_error";
    }
}

### string constants for Ghostscript run
# get Ghostscript command name
$::opt_gscmd = '';
sub find_ghostscript () {
    return if $::opt_gscmd;
    if ($::opt_debug) {
        print "* Perl executable: $^X\n";
        if ($] < 5.006) {
            print "* Perl version: $]\n";
        }
        else {
            printf "* Perl version: v%vd\n", $^V;
        }
        if (defined &ActivePerl::BUILD) {
            printf "* Perl product: ActivePerl, build %s\n", ActivePerl::BUILD();
        }
        use Config;
        printf "* Pointer size: $Config{'ptrsize'}\n";
        printf "* Pipe support: %s\n",
                (defined($Config{'d_pipe'}) ? 'yes' : 'no');
        printf "* Fork support: %s\n",
                (defined($Config{'d_fork'}) ? 'yes' : 'no');
    }
    my $system = 'unix';
    $system = "dos" if $^O =~ /dos/i;
    $system = "os2" if $^O =~ /os2/i;
    $system = "win" if $^O =~ /mswin32/i;
    $system = "cygwin" if $^O =~ /cygwin/i;
    $system = "miktex" if defined($ENV{"TEXSYSTEM"}) and
                          $ENV{"TEXSYSTEM"} =~ /miktex/i;
    print "* OS name: $^O\n" if $::opt_debug;
    print "* Arch name: $archname\n" if $::opt_debug;
    print "* System: $system\n" if $::opt_debug;
    my %candidates = (
        'unix' => [qw|gs gsc|],
        'dos' => [qw|gs386 gs|],
        'os2' => [qw|gsos2 gs|],
        'win' => [qw|gswin32c gs|],
        'cygwin' => [qw|gs gswin32c|],
        'miktex' => [qw|mgs gswin32c gs|]
    );
    if ($system eq 'win' or $system eq 'cygwin' or $system eq 'miktex') {
        if ($archname =~ /mswin32-x64/i) {
            my @a = ();
            foreach my $name (@{$candidates{$system}}) {
                push @a, 'gswin64c' if $name eq 'gswin32c';
                push @a, $name;
            }
            $candidates{$system} = \@a;
        }
    }
    my %ext = (
        'unix' => '',
        'dos' => '.exe',
        'os2' => '.exe',
        'win' => '.exe',
        'cygwin' => '.exe',
        'miktex' => '.exe'
    );
    my $candidates_ref = $candidates{$system};
    my $ext = $Config{'_exe'};
    $ext = $ext{$system} unless defined $ext;
    use File::Spec;
    my @path = File::Spec->path();
    my $found = 0;
    foreach my $candidate (@$candidates_ref) {
        foreach my $dir (@path) {
            my $file = File::Spec->catfile($dir, "$candidate$ext");
            if (-x $file) {
                $::opt_gscmd = $candidate;
                $found = 1;
                print "* Found ($candidate): $file\n" if $::opt_debug;
                last;
            }
            print "* Not found ($candidate): $file\n" if $::opt_debug;
        }
        last if $found;
    }
    if (not $found and $Win) {
        $found = SearchRegistry();
    }
    if ($found) {
        print "* Autodetected ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
    else {
        $::opt_gscmd = $$candidates_ref[0];
        print "* Default ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
}

sub SearchRegistry () {
    my $found = 0;
    eval 'use Win32::TieRegistry qw|KEY_READ REG_SZ|;';
    if ($@) {
        if ($::opt_debug) {
            print "* Registry lookup for Ghostscript failed:\n";
            my $msg = $@;
            $msg =~ s/\s+$//;
            foreach (split /\r?\n/, $msg) {
                print "  $_\n";
            }
        }
        return $found;
    }
    my $open_params = {Access => KEY_READ(), Delimiter => '/'};
    my $key_name_software = 'HKEY_LOCAL_MACHINE/SOFTWARE/';
    my $current_key = $key_name_software;
    my $software = new Win32::TieRegistry $current_key, $open_params;
    if (not $software) {
        print "* Cannot find or access registry key `$current_key'!\n"
                if $::opt_verbose;
        return $found;
    }
    print "* Search registry at `$current_key'.\n" if $::opt_debug;
    my %list;
    foreach my $key_name_gs (grep /Ghostscript/i, $software->SubKeyNames()) {
        $current_key = "$key_name_software$key_name_gs/";
        print "* Registry entry found: $current_key\n" if $::opt_debug;
        my $key_gs = $software->Open($key_name_gs, $open_params);
        if (not $key_gs) {
            print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
            next;
        }
        foreach my $key_name_version ($key_gs->SubKeyNames()) {
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            print "* Registry entry found: $current_key\n" if $::opt_debug;
            if (not $key_name_version =~ /^(\d+)\.(\d+)$/) {
                print "  The sub key is not a version number!\n" if $::opt_debug;
                next;
            }
            my $version_main = $1;
            my $version_sub = $2;
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            my $key_version = $key_gs->Open($key_name_version, $open_params);
            if (not $key_version) {
                print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
                next;
            }
            $key_version->FixSzNulls(1);
            my ($value, $type) = $key_version->GetValue('GS_DLL');
            if ($value and $type == REG_SZ()) {
                print "  GS_DLL = $value\n" if $::opt_debug;
                $value =~ s|([\\/])([^\\/]+\.dll)$|$1gswin32c.exe|i;
                my $value64 = $value;
                $value64 =~ s/gswin32c\.exe$/gswin64c.exe/;
                if ($archname =~ /mswin32-x64/i and -f $value64) {
                    $value = $value64;
                }
                if (-f $value) {
                    print "  EXE found: $value\n" if $::opt_debug;
                }
                else {
                    print "  EXE not found!\n" if $::opt_debug;
                    next;
                }
                my $sortkey = sprintf '%02d.%03d %s',
                        $version_main, $version_sub, $key_name_gs;
                $list{$sortkey} = $value;
            }
            else {
                print "  Missing key `GS_DLL' with type `REG_SZ'!\n" if $::opt_debug;
            }
        }
    }
    foreach my $entry (reverse sort keys %list) {
        $::opt_gscmd = $list{$entry};
        print "* Found (via registry): $::opt_gscmd\n" if $::opt_debug;
        $found = 1;
        last;
    }
    return $found;
}

# restricted mode
my $restricted = 0;
if ($0 =~ /rpdfcrop/ or $0 =~ /restricted/) {
    $restricted = 1;
}

# "null" device
use File::Spec::Functions qw(devnull);
my $null = devnull();

### variables
my $inputfile   = "";
my $outputfile  = "";
my $tmp = "tmp-\L$program\E-$$";

### paper sizes

my @papersizes = qw[
  11x17 ledger legal letter lettersmall
  archE archD archC archB archA
  a0 a1 a2 a3 a4 a4small a5 a6 a7 a8 a9 a10
  isob0 isob1 isob2 isob3 isob4 isob5 isob6
  c0 c1 c2 c3 c4 c5 c6
  jisb0 jisb1 jisb2 jisb3 jisb4 jisb5 jisb6
  b0 b1 b2 b3 b4 b5
  flsa flse halfletter
];
my %papersizes;
foreach (@papersizes) {
    $papersizes{$_} = 1;
}

### option variables
my @bool = ("false", "true");
$::opt_version    = 0;
$::opt_help       = 0;
$::opt_debug      = 0;
$::opt_verbose    = 0;
$::opt_pdftexcmd  = "pdftex";
$::opt_xetexcmd   = "xetex";
$::opt_luatexcmd  = "luatex";
$::opt_tex        = "pdftex";
$::opt_margins    = "0 0 0 0";
$::opt_clip       = 0;
$::opt_hires      = 0;
$::opt_papersize  = "";
$::opt_resolution = "";
$::opt_bbox       = "";
$::opt_bbox_odd   = "";
$::opt_bbox_even  = "";
$::opt_initex     = 0;
$::opt_pdfversion = "auto";

sub usage ($) {
    my $ret = shift;
    find_ghostscript();
    my $usage = <<"END_OF_USAGE";
${title}Syntax:   \L$program\E [options] <input[.pdf]> [output file]
Function: Margins are calculated and removed for each page in the file.
Options:                                                       (defaults:)
  --help              print usage
  --version           print version number
  --(no)verbose       verbose printing                         ($bool[$::opt_verbose])
  --(no)debug         debug informations                       ($bool[$::opt_debug])
  --gscmd <name>      call of ghostscript                      ($::opt_gscmd)
  --pdftex | --xetex | --luatex
                      use pdfTeX | use XeTeX | use LuaTeX      ($::opt_tex)
  --pdftexcmd <name>  call of pdfTeX                           ($::opt_pdftexcmd)
  --xetexcmd <name>   call of XeTeX                            ($::opt_xetexcmd)
  --luatexcmd <name>  call of LuaTeX                           ($::opt_luatexcmd)
  --margins "<left> <top> <right> <bottom>"                    ($::opt_margins)
                      add extra margins, unit is bp. If only one number is
                      given, then it is used for all margins, in the case
                      of two numbers they are also used for right and bottom.
  --(no)clip          clipping support, if margins are set     ($bool[$::opt_clip])
                      (not available for --xetex)
  --(no)hires         using `%%HiResBoundingBox'               ($bool[$::opt_hires])
                      instead of `%%BoundingBox'
  --(no)ini           use iniTeX variant of the TeX compiler   ($bool[$::opt_initex])
Expert options:
  --restricted        turn on restricted mode                  ($bool[$restricted])
  --papersize <foo>   parameter for gs's -sPAPERSIZE=<foo>,
                      use only with older gs versions <7.32    ($::opt_papersize)
  --resolution <xres>x<yres>                                   ($::opt_resolution)
  --resolution <res>  pass argument to ghostscript's option -r
                      Example: --resolution 72
  --bbox "<left> <bottom> <right> <top>"                       ($::opt_bbox)
                      override bounding box found by ghostscript
                      with origin at the lower left corner
  --bbox-odd          Same as --bbox, but for odd pages only   ($::opt_bbox_odd)
  --bbox-even         Same as --bbox, but for even pages only  ($::opt_bbox_even)
  --pdfversion <1.x> | auto | none
                      Set the PDF version to 1.x, 1 < x < 8.
                      If `auto' is given as value, then the
                      PDF version is taken from the header
                      of the input PDF file.
                      An empty value or `none' uses the
                      default of the TeX engine.               ($::opt_pdfversion)

Input file: If the name is `-', then the standard input is used and
  the output file name must be explicitly given.
Examples:
  \L$program\E --margins 10 input.pdf output.pdf
  \L$program\E --margins '5 10 5 20' --clip input.pdf output.pdf
In case of errors:
  Try option --verbose first to get more information.
In case of bugs:
  Please, use option --debug for bug reports.
END_OF_USAGE
    if ($ret) {
        die $usage;
    }
    else {
        print $usage;
        exit(0);
    }
}

### process options
my @OrgArgv = @ARGV;
use Getopt::Long;
GetOptions(
  "help!",
  "version!",
  "debug!",
  "verbose!",
  "gscmd=s",
  "pdftexcmd=s",
  "xetexcmd=s",
  "luatexcmd=s",
  "pdftex" => sub { $::opt_tex = 'pdftex'; },
  "xetex"  => sub { $::opt_tex = 'xetex'; },
  "luatex" => sub { $::opt_tex = 'luatex'; },
  "initex!",
  "margins=s",
  "clip!",
  "hires!",
  "papersize=s",
  "resolution=s",
  "bbox=s",
  "bbox-odd=s" => \$::opt_bbox_odd,
  "bbox-even=s" => \$::opt_bbox_even,
  "restricted" => sub { $restricted = 1; },
  "pdfversion=s" => \$::opt_pdfversion,
) or usage(1);
!$::opt_help or usage(0);

if ($::opt_version) {
    print "$prj $date v$version\n";
    exit(0);
}

$::opt_verbose = 1 if $::opt_debug;

@ARGV >= 1 or usage(1);

print $title;

print "* Restricted mode: ", ($restricted ? "enabled" : "disabled"), "\n"
        if $::opt_debug;

$::opt_pdfversion =~ /^(|none|auto|1\.([2-7]))$/
        or die "!!! Error: Invalid value `$::opt_pdfversion' for option `--pdfversion'!\n";
print "* Option `pdfversion': $::opt_pdfversion\n" if $::opt_debug;
$::opt_pdfversion = $2 if $2;
$::opt_pdfversion = '' if $::opt_pdfversion eq 'none';

find_ghostscript();

if ($::opt_bbox) {
    $::opt_bbox =~ s/^\s+//;
    $::opt_bbox =~ s/\s+$//;
    $::opt_bbox =~ s/\s+/ /;
    if ($::opt_bbox =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box: $::opt_bbox\n" if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox \"$::opt_bbox\")!\n";
    }
}
if ($::opt_bbox_odd) {
    $::opt_bbox_odd =~ s/^\s+//;
    $::opt_bbox_odd =~ s/\s+$//;
    $::opt_bbox_odd =~ s/\s+/ /;
    if ($::opt_bbox_odd =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for odd pages: $::opt_bbox_odd\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-odd \"$::opt_bbox_odd\")!\n";
    }
}
if ($::opt_bbox_even) {
    $::opt_bbox_even =~ s/^\s+//;
    $::opt_bbox_even =~ s/\s+$//;
    $::opt_bbox_even =~ s/\s+/ /;
    if ($::opt_bbox_even =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for even pages: $::opt_bbox_even\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-even \"$::opt_bbox_even\")!\n";
    }
}

@ARGV <= 2 or die "$Error Too many files!\n";

### input file
$inputfile = shift @ARGV;

if ($inputfile eq '-') {
    @ARGV == 1 or die "$Error Missing output file name!\n";
    print "* Input file: <stdin>\n" if $::opt_debug;
}
else {
    if (! -f $inputfile) {
        if (-f "$inputfile.pdf") {
            $inputfile .= ".pdf";
        }
        else {
            die "$Error Input file `$inputfile' not found!\n";
        }
    }
    print "* Input file: $inputfile\n" if $::opt_debug;
}

### output file
if (@ARGV) {
    $outputfile = shift @ARGV;
}
else {
    $outputfile = $inputfile;
    $outputfile =~ s/\.pdf$//i;
    $outputfile .= "-crop.pdf";
}

print "* Output file: $outputfile\n" if $::opt_debug;

### margins
my ($llx, $lly, $urx, $ury) = (0, 0, 0, 0);
if ($::opt_margins =~
        /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
    ($llx, $lly, $urx, $ury) = ($1, $2, $3, $4);
}
else {
    if ($::opt_margins =~ /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
        ($llx, $lly, $urx, $ury) = ($1, $2, $1, $2);
    }
    else {
        if ($::opt_margins =~ /^\s*([\-\.\d]+)\s*$/) {
            ($llx, $lly, $urx, $ury) = ($1, $1, $1, $1);
        }
        else {
            die "$Error Parse error (option --margins)!\n";
        }
    }
}
print "* Margins: $llx $lly $urx $ury\n" if $::opt_debug;

### papersize validation (security)
if ($::opt_papersize ne '') {
    $::opt_papersize =~ /^[0-9A-Za-z]+$/
            or die "$Error Invalid papersize ($::opt_papersize)!\n";
    $papersizes{$::opt_papersize}
            or die "$Error Unknown papersize ($::opt_papersize),"
                   . " see ghostscript's documentation for option `-r'!\n";
}

### resolution validation (security)
if ($::opt_resolution ne '') {
    $::opt_resolution =~ /^\d+(x\d+)?$/
            or die "$Error Invalid resolution ($::opt_resolution),"
                   . " see ghostscript's documentation!\n";
}

### command name validation (security)
my %cmd = (
    'gscmd' => \$::opt_gscmd,
    'pdftexcmd' => \$::opt_pdftexcmd,
    'luatexcmd' => \$::opt_luatexcmd,
    'xetexcmd' => \$::opt_xetexcmd
);
foreach my $cmd (keys %cmd) {
    my $cmd_ref = $cmd{$cmd};
    $$cmd_ref =~ s/^\s+//;
    $$cmd_ref =~ s/\s+$//;
    my $val = $$cmd_ref;
    next unless $val;
    next unless $val;
    if ($val =~ /`/) {
        die "$Error Forbidden backtick for option `--$cmd' ($val)!\n";
    }
    if ($val =~ /\s/) {
        my $err = 0;
        if ($restricted or not $Win) {
            $err = 1;
        }
        else {
            $err = 1 if $val =~ /\.exe.*\s/i;
            $err = 1 if $val =~ /\s[-\/@+]/;
        }
        die "$Error Forbidden whitespace for option `--$cmd' ($val)!\n" if $err;
    }
}
if ($restricted) {
    if ($::opt_pdftexcmd and $::opt_pdftexcmd ne 'pdftex') {
        die "$Error pdfTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_xetexcmd and $::opt_xetexcmd ne 'xetex') {
        die "$Error XeTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_luatexcmd and $::opt_luatexcmd ne 'luatex') {
        die "$Error LuaTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_gscmd) {
        $::opt_gscmd =~ /^(gs|mgs|gswin32c|gs386|gsos2)$/
        or $::opt_gscmd =~ /^gs[\-_]?(\d|\d[\.-_]?\d\d)c?$/
        or die "$Error: Invalid Ghostscript program name in restricted mode!\n";
    }
}
if ($Win and $::opt_gscmd =~ /\s/) {
    $::opt_gscmd = "\"$::opt_gscmd\"";
}

### cleanup system
my @unlink_files = ();
my $exit_code = 1;
sub clean {
    print "* Cleanup\n" if $::opt_debug;
    if ($::opt_debug) {
        print "* Temporary files: @unlink_files\n";
    }
    else {
        for (; @unlink_files>0; ) {
            unlink shift @unlink_files;
        }
    }
}
sub cleanup {
    clean();
    exit($exit_code);
}
$SIG{'INT'} = \&cleanup;
$SIG{'__DIE__'} = \&clean;

### Calculation of BoundingBoxes

# use safe file name for use within cmd line of gs (unknown shell: space, ...)
# and XeTeX (hash, curly braces, ...)
my $inputfilesafe = $inputfile;
if ($inputfile eq '-') {
    $inputfilesafe = "$tmp-stdin.pdf";
    print "* Temporary input file: $inputfilesafe\n" if $::opt_debug;
    push @unlink_files, $inputfilesafe;
    open(OUT, '>', $inputfilesafe)
            or die sprintf "$Error Cannot write `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    binmode(OUT);
    my $size = 0;
    my $len = 0;
    my $buf = '';
    my $buf_size = 65536;
    do {
        $len = read STDIN, $buf, $buf_size;
        if (not defined $len) {
            my $msg = exterr;
            die "$Error Reading standard input ($msg)!\n";
        }
        print OUT $buf
                or die sprintf "$Error Writing `%s` (%s)!\n",
                               $inputfilesafe, exterr;
        $size += $len;
    }
    while ($len);
    close(OUT);
    print "* File size (STDIN): $size\n" if $::opt_debug;
}
elsif (not $inputfile =~ /^[\w\d\.\-\:\/@]+$/) { # /[\s\$~'"#{}%]/
    $inputfilesafe = "$tmp-img.pdf";
    push @unlink_files, $inputfilesafe;
    my $symlink_exists = eval {
        local $SIG{'__DIE__'};
        symlink("", "");
        1;
    };
    print "* Input file name `$inputfile' contains special characters.\n"
          . "* " . ($symlink_exists ? "Link" : "Copy")
          . " input file to temporary file `$inputfilesafe'.\n"
            if $::opt_verbose;
    if ($symlink_exists) {
        symlink($inputfile, $inputfilesafe)
            or die sprintf "$Error Link from `%s' to `%s' failed (%s)!\n",
                           $inputfile, $inputfilesafe, exterr;
    }
    else {
        use File::Copy;
        copy($inputfile, $inputfilesafe)
                or die sprintf "$Error Copy from `%s' to `%s' failed (%s)\n",
                               $inputfile, $inputfilesafe, exterr;
    }
}

if ($::opt_pdfversion eq 'auto') {
    open(IN, '<', $inputfilesafe)
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    my $buf;
    read(IN, $buf, 1024)
            or die sprintf "!!! Error: Cannot read the header of `%s' failed (%s)!\n",
                           $inputfilesafe, exterr;
    close(IN);
    if ($buf =~ /%PDF-1.([0-7])\s/) {
        $::opt_pdfversion = $1;
        print "* PDF header: %PDF-1.$::opt_pdfversion\n" if $::opt_verbose;
        $::opt_pdfversion = 2 if $::opt_pdfversion < 2;
    }
    else {
        die "!!! Error: Cannot find PDF header of `$inputfilesafe'!\n";
    }
}
print '* Using PDF minor version: ',
      ($::opt_pdfversion ? $::opt_pdfversion : "engine's default"),
      "\n" if $::opt_debug;

my @gsargs = (
    "-sDEVICE=bbox",
    "-dBATCH",
    "-dNOPAUSE"
);
push @gsargs, "-sPAPERSIZE=$::opt_papersize" if $::opt_papersize;
push @gsargs, "-r$::opt_resolution" if $::opt_resolution;
push @gsargs,
    "-c",
    "save",
    "pop",
    "-f",
    $inputfilesafe
;

my $tmpfile = "$tmp.tex";
push @unlink_files, $tmpfile;
open(TMP, ">$tmpfile")
    or die sprintf "$Error Cannot write tmp file `%s' (%s)!\n",
                   $tmpfile, exterr;
print TMP <<'END_TMP';
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
END_TMP
my $pdffilehex = unpack 'H*', $inputfilesafe;
$pdffilehex = "\U$pdffilehex\E";
print TMP "\\def\\pdffilehex{$pdffilehex}\n";
print TMP <<'END_TMP';
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
END_TMP
if ($::opt_tex eq 'luatex') {
    print TMP <<'END_TMP';
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
  \errmessage{LuaTeX not found!}%
\else
  \begingroup
    \newlinechar=10 %
    \endlinechar=\newlinechar %
    \ifnum0%
        \directlua{%
          if tex.enableprimitives then
            tex.enableprimitives('TEST', {
              'luatexversion',
              'pdfoutput',
              'pdfcompresslevel',
              'pdfhorigin',
              'pdfvorigin',
              'pdfpagewidth',
              'pdfpageheight',
              'pdfmapfile',
              'pdfximage',
              'pdflastximage',
              'pdfrefximage',
              'pdfminorversion',
              'pdfobjcompresslevel',
            })
            tex.print('1')
          end
        }%
        \ifx\TESTluatexversion\UnDeFiNeD\else 1\fi %
        =11 %
      \global\let\luatexversion\luatexversion %
      \global\let\pdfoutput\TESTpdfoutput %
      \global\let\pdfcompresslevel\TESTpdfcompresslevel %
      \global\let\pdfhorigin\TESTpdfhorigin %
      \global\let\pdfvorigin\TESTpdfvorigin %
      \global\let\pdfpagewidth\TESTpdfpagewidth %
      \global\let\pdfpageheight\TESTpdfpageheight %
      \global\let\pdfmapfile\TESTpdfmapfile %
      \global\let\pdfximage\TESTpdfximage %
      \global\let\pdflastximage\TESTpdflastximage %
      \global\let\pdfrefximage\TESTpdfrefximage %
      \global\let\pdfminorversion\TESTpdfminorversion %
      \global\let\pdfobjcompresslevel\TESTpdfobjcompresslevel %
    \else %
      \errmessage{%
        Missing \string\luatexversion %
      }%
    \fi %
  \endgroup %
\fi
END_TMP
}
if ($::opt_tex eq 'pdftex' or $::opt_tex eq 'luatex') {
    print TMP <<'END_TMP_HEAD';
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
END_TMP_HEAD
    print TMP "\\setpdfversion{$::opt_pdfversion}\n" if $::opt_pdfversion;
}
else { # XeTeX
    print TMP <<'END_TMP_HEAD';
\expandafter\ifx\csname XeTeXpdffile\endcsname\relax
  \errmessage{XeTeX not found or too old!}%
\fi
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \shipout\hbox{%
    \kern-1in%
    \kern-#2bp%
    \vbox{%
      \kern-1in%
      \kern#3bp%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \page {#1} [#2 #3 #4 #5]%
}
\def\pageinclude#1{%
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \kern-1in%
    \vbox{%
      \kern-1in%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
END_TMP_HEAD
}

print "* Running ghostscript for BoundingBox calculation ...\n"
    if $::opt_verbose;
print "* Ghostscript call: $::opt_gscmd @gsargs\n" if $::opt_debug;

my @bbox;
my @bbox_all;
my @bbox_odd;
my @bbox_even;
if ($::opt_bbox) {
     $::opt_bbox =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_all = ($1, $2, $3, $4);
}
if ($::opt_bbox_odd) {
     $::opt_bbox_odd =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_odd = ($1, $2, $3, $4);
}
if ($::opt_bbox_even) {
     $::opt_bbox_even =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_even = ($1, $2, $3, $4);
}

sub getbbox ($$$$$) {
    my $page = shift;
    my $a = shift;
    my $b = shift;
    my $c = shift;
    my $d = shift;
    if ($page % 2 == 1) {
        if ($::opt_bbox_odd) {
            return @bbox_odd;
        }
    }
    else {
        if ($::opt_bbox_even) {
            return @bbox_even;
        }
    }
    if ($::opt_bbox) {
        return @bbox_all;
    }
    return ($a, $b, $c, $d);
}
my $page = 0;
my $gs_pipe = "$::opt_gscmd -dSAFER @gsargs 2>&1";
$gs_pipe .= " 1>$null" unless $::opt_verbose;
$gs_pipe .= " |";

open(GS, $gs_pipe)
        or die sprintf "$Error Cannot call ghostscript `%s' (%s)!\n",
                       $::opt_gscmd, exterr;
my $bb = ($::opt_hires) ? "%%HiResBoundingBox" : "%%BoundingBox";
my $previous_line = 'Previous line';
# Ghostscript workaround for buggy ports that prints
# the bounding box data twice on STDERR.
while (<GS>) {
    print $_ if $::opt_verbose;
    if (/^$bb:\s*(-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+)/o) {
    }
    else {
        $previous_line = $_;
        next;
    }
    next if $previous_line eq $_;
    $previous_line = $_;
    $page++;
    @bbox = getbbox($page, $1, $2, $3, $4);

    my $empty = 0;
    $empty = 1 if $bbox[0] >= $bbox[2];
    $empty = 1 if $bbox[1] >= $bbox[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: Empty Bounding Box is returned by Ghostscript!
!!!   Page $page: @bbox
!!! Either there is a problem with the page or with Ghostscript.
!!! Recovery is tried by embedding the page in its original size.

END_WARNING
        print TMP "\\pageinclude{$page}\n";
        next;
    }

    print "* Page $page: @bbox\n" if $::opt_verbose;

    my @bb = ($bbox[0] - $llx, $bbox[1] - $ury,
             $bbox[2] + $urx, $bbox[3] + $lly);

    $empty = 0;
    $empty = 1 if $bb[0] >= $bb[2];
    $empty = 1 if $bb[1] >= $bb[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: The final Bounding Box is empty!
!!!   Page: $page: @bb
!!! Probably caused by too large negative margin values.
!!! Recovery by ignoring margin values.

END_WARNING
        print TMP "\\page $page [@bbox]\n";
        # clipping shouldn't make a difference
        next;
    }
    if ($::opt_clip) {
        print TMP "\\pageclip $page [@bbox][$llx $lly $urx $ury]\n";
    }
    else {
        print TMP "\\page $page [@bb]\n";
    }
}
close(GS);

if ($? == -1) {
    die sprintf "$Error Ghostscript failed to execute (%s)!\n",
                exterr;
}
elsif ($? & 127) {
    die sprintf  "$Error Ghostscript died with signal %d!\n",
                 ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error Ghostscript exited with error code %d!\n",
                $? >> 8;
}

print TMP "\\csname \@\@end\\endcsname\n\\end\n";
close(TMP);

if ($page == 0) {
    die "$Error Ghostscript does not report bounding boxes!\n";
}

### Run pdfTeX/XeTeX

push @unlink_files, "$tmp.log";
my $cmd;
my $texname;
if ($::opt_tex eq 'pdftex') {
    $cmd = $::opt_pdftexcmd;
    $texname = 'pdfTeX';
}
elsif ($::opt_tex eq 'luatex') {
    $cmd = $::opt_luatexcmd;
    $texname = 'LuaTeX';
}
else {
    $cmd = $::opt_xetexcmd;
    $texname = 'XeTeX';
}
$cmd = "\"$cmd\"" if $Win and $cmd =~ /\s/;
$cmd .= ' -no-shell-escape';
if ($::opt_initex) {
    $cmd .= ' --ini --etex';
}
if ($::opt_verbose) {
    $cmd .= " -interaction=nonstopmode $tmp";
}
else {
    $cmd .= " -interaction=batchmode $tmp";
}
print "* Running $texname ...\n" if $::opt_verbose;
print "* $texname call: $cmd\n" if $::opt_debug;
if ($::opt_verbose) {
    system($cmd);
}
else {
    `$cmd`;
}
if ($? == -1) {
    die sprintf "$Error %s run failed to execute (%s)!\n",
                $texname, exterr;
}
elsif ($? & 127) {
    die sprintf "$Error %s run died with signal %d!\n",
                $texname, ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error %s run failed with value %d!\n",
                $texname, ($? >> 8);
}

### Check pdf version of temp file
if ($::opt_pdfversion) {
    open(PDF, '+<', "$tmp.pdf")
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    my $header;
    read PDF, $header, 9
            or die sprintf "!!! Error: Cannot read header of `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    $header =~ /^%PDF-1\.(\d)\s$/ or die "!!! Error: Cannot find header of `$tmp.pdf'!\n";
    if ($1 ne $::opt_pdfversion) {
        seek PDF, 7, 0
                or die sprintf "!!! Error: Cannot seek in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print PDF $::opt_pdfversion
                or die sprintf "!!! Error: Cannot write in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print "* PDF version correction in output file: 1.$::opt_pdfversion\n"
                if $::opt_debug;
    }
    close(PDF);
}

### Move temp file to output
if (!rename("$tmp.pdf", $outputfile)) {
    use File::Copy;
    move "$tmp.pdf", $outputfile or
            die "$Error Cannot move `$tmp.pdf' to `$outputfile'!\n";
}

print "==> $page page", (($page == 1) ? "" : "s"),
      " written on `$outputfile'.\n";

$exit_code = 0;
cleanup();

__END__


==> tab-ablationNumLayers.tex <==
% !TeX root = main.tex
\begin{table}[h]
	\centering
	\includegraphics[width=\textwidth{}]{figs/placeholder-ablation_num_layers.pdf}
%	\vspace{-2em}
	\caption{efficacy of the number of proxy model layers}
	\label{tab:ablationNumLayers}
%	\vspace{-2em}
\end{table}

==> tab-approxsaving.tex <==
% !TeX root = main.tex
\begin{table}
    \centering
    \caption{Accuracy and cost influence arch}
    \includegraphics[width=0.4\textwidth{}]{figs/placeholder-approxsaving.png}
    \label{tab:collision}
\end{table}


==> tab-introresults.tex <==
% !TeX root = main.tex
\begin{table}[t]
		\includegraphics[width=0.48\textwidth{}]{figs/placeholder-intro.png}
		\caption{results put in the first page}
		\label{tab:network-confs}
\end{table}

==> tab-phaseproxyconfig.tex <==
% !TEX root = main.tex
\begin{table}[t]
	\centering
	\caption{
		configurations
	}
	\includegraphics[width=0.48\textwidth{}]{figs/placeholder-phaseproxyconfig.png}
%	\vspace{-2em}
	\label{tab:config}
%	\vspace{-3em}
\end{table}

==> tab-transformer-analysis.tex <==
% !TeX root = main.tex

% \begin{table}[t]
% 	\centering
% \includegraphics[width=0.8\textwidth{}]{figs/tab-transformer-analysis.pdf}
% 	\caption{
% 	Evaluating Transformers over MPC incurs high communication and computation overhead. 
% 	The measurement is for one forward pass of one Transformer layer (12 heads) over a batch of 5 data points (maximum allowable on GPU memory). For activation, we use RELU. Hardware: Nvidia Quadro RTX 4000. MPC framework: Crypten~\cite{knott2021crypten}. 
% 	}
% 	\label{fig:design:transformer-analysis}
% \end{table}

\begin{wrapfigure}{r}{0cm}
\includegraphics[width=0.4\textwidth{}]{figs/tab-transformer-analysis.pdf}
% \vspace{-2em}
    \caption{Transformers over MPC incurs high communication and computation overhead. 
	Showing one forward pass of one layer (12 heads) over a batch of 5 (maximum allowable on our GPU). Hardware: Quadro RTX 4000. MPC framework: Crypten~\cite{knott2021crypten}. }
    \label{tab:transformer-analysis}
    % \vspace{-1em}
\end{wrapfigure} 
